Watch Your Back: Identifying Cybercrime Financial Relationships in Bitcoin through Back-and-Forth Exploration

Cybercriminals often leverage Bitcoin for their illicit activities. In this work, we propose back-and-forth exploration, a novel automated Bitcoin transaction tracing technique to identify cybercrime financial relationships. Given seed addresses belonging to a cybercrime campaign, it outputs a transaction graph, and identifies paths corresponding to relationships between the campaign under study and external services and other cybercrime campaigns. Back-and-forth exploration provides two key contributions. First, it explores both forward and backwards, instead of only forward as done by prior work, enabling the discovery of relationships that cannot be found by only exploring forward (e.g., deposits from clients of a mixer). Second, it prevents graph explosion by combining a tagging database with a machine learning classifier for identifying addresses belonging to exchanges. We evaluate back-and-forth exploration on 30 malware families. We build oracles for 4 families using Bitcoin for C&C and use them to demonstrate that back-and-forth exploration identifies 13 C&C signaling addresses missed by prior work, 8 of which are fundamentally missed by forward-only explorations. Our approach uncovers a wealth of services used by the malware including 44 exchanges, 11 gambling sites, 5 payment service providers, 4 underground markets, 4 mining pools, and 2 mixers. In 4 families, the relations include new attribution points missed by forward-only explorations. It also identifies relationships between the malware families and other cybercrime campaigns, highlighting how some malware operators participate in a variety of cybercriminal activities.

==> Makefile <==
PROJECT=paper

# xfig documents whose corresponding EPS fies are used in the paper
# FIGFILES = segment.fig allocGroup.fig

# matlab scripts that generate output for the paper. These are *.m files
# that generate a corresponding *.eps file when run.
MFILES =

# GNUplot files
PLTFILES = 

# Other EPS files that are necessary to build the document
# If you have eps files that you generate by hand, list them here.
EPSFILES =

# Non-refdbms bib files to be included
# If you need a local .bib file, put that here.
LOCALBIB = bibliography/paper.bib
LOCALXTXBIB = bibliography/paper.xtx

# default targets to make for make all
TARGETS = $(PROJECT).pdf
TARGETSPS = $(PROJECT).ps

#-- Programs used when runing latex etc.                       
BIBTEX = bibtex
XTEX = crosstex
LATEX = latex
DVIPS = dvips -tletter
FIG2DEV = fig2dev
MATLAB = matlab
GNUPLOT = gnuplot
PS2PDF = ps2pdf
PDFLATEX = pdflatex

SRCFILES = $(wildcard *.tex)
EPSFIGFILES = $(FIGFILES:.fig=.eps)
EPSMFILES = $(MFILES:.m=.eps)
EPSPLTFILES = $(PLTFILES:.plt=.eps)
EPSFILES += $(EPSFIGFILES) $(EPSMFILES) $(EPSPLTFILES)

#--------------------------------------------------------------------------
# Production/target rules                       
#--------------------------------------------------------------------------
.SUFFIXES:
.PHONY: clean all veryclean
#-- EPS files may be expensive to regenerate, so keep them even though they
#-- are intermediate targets
.PRECIOUS: $(EPSMFILES) $(EPSFIGFILES)
#.PRECIOUS: $(EPSMFILES)

all: $(TARGETS)

#-- Make EPS files from matlab documents
%.eps: %.m
	$(MATLAB) -nodesktop -r "$*;quit" || $(MATLAB) -nodisplay -r "$*;quit"

#-- Make EPS files from xfig documents
%.eps: %.fig
	$(FIG2DEV) -L eps $< $@ || $(FIG2DEV) -L ps $< $@

#-- Make EPS files from GNUplot scripts
%.eps: %.plt
	$(GNUPLOT) $<

#-- Creation of initial .aux file
%.aux: %.tex $(SRCFILES) $(EPSFILES)
	$(LATEX) $<

#-- Create .bbl from .bib
%.bbl: %.aux $(LOCALBIB)
	$(BIBTEX) $*
	$(LATEX) $*.tex
	$(LATEX) $*.tex

#-- Build a dvi... 
#%.dvi: %.tex %.bbl $(EPSFILES) $(LOCALBIB)
%.dvi: %.tex %.bbl
	$(LATEX) $<

#-- converting .dvi to .ps... requires the EPS files
%.ps: %.dvi $(EPSFILES)
	$(DVIPS) -o $@ $<

#-- converting .ps to .pdf.
#%.pdf: %.ps
#	$(PS2PDF) $<

#-- generating pdf using pdflatex
%.pdf: %.tex $(SRCFILES) $(LOCALBIB)
	$(PDFLATEX) $*
#	$(BIBTEX) $*
#	$(PDFLATEX) $*
#	$(BIBTEX) $*
#	$(PDFLATEX) $*
	chmod +x $*.pdf

full: $(SRCFILES) $(LOCALBIB)
	$(PDFLATEX) $(PROJECT)
	$(BIBTEX) $(PROJECT)
	$(PDFLATEX) $(PROJECT)
	$(BIBTEX) $(PROJECT)
	$(PDFLATEX) $(PROJECT)
	chmod +x $(PROJECT).pdf
	

bib:	$(LOCALXTXBIB)
	$(XTEX) --short=state --short=conference --no-field editor --no-field publisher \
		--no-field pages --xtx2bib $(LOCALXTXBIB)

ps:	$(TARGETSPS)

pdf:
	$(PS2PDF) $(TARGETS)

clean:
	rm -f *~  $(TARGETS) $(TARGETSPS) *.dvi *.log *.aux *.blg *.bbl $(OLDAUX)

veryclean: clean
	rm -f $(EPSFIGFILES) $(EPSMFILES) $(EPSPLTFILES)

spell:	$(SRCFILES)
	detex $^ | spell | env LANG=C sort -u | env LANG=C comm -23 - ok-words

